Low-rank tensor reconstruction of concentrated densities with application to Bayesian inversion

Transport maps have become a popular mechanic to express complicated probability densities using sample propagation through an optimized push-forward. Beside their broad applicability and well-known success, transport maps suffer from several drawbacks such as numerical inaccuracies induced by the optimization process and the fact that sampling schemes have to be employed when quantities of interest, e.g. moments are to compute. This paper presents a novel method for the accurate functional approximation of probability density functions (PDF) that copes with those issues. By interpreting the pull-back result of a target PDF through an inexact transport map as a perturbed reference density, a subsequent functional representation in a more accessible format allows for efficient and more accurate computation of the desired quantities. We introduce a layer-based approximation of the perturbed reference density in an appropriate coordinate system to split the high-dimensional representation problem into a set of independent approximations for which separately chosen orthonormal basis functions are available. This effectively motivates the notion of h- and p-refinement (i.e. ``mesh size'' and polynomial degree) for the approximation of high-dimensional PDFs. To circumvent the curse of dimensionality and enable sampling-free access to certain quantities of interest, a low-rank reconstruction in the tensor train format is employed via the Variational Monte Carlo method. An a priori convergence analysis of the developed approach is derived in terms of Hellinger distance and the Kullback-Leibler divergence. Applications comprising Bayesian inverse problems and several degrees of concentrated densities illuminate the (superior) convergence in comparison to Monte Carlo and Markov-Chain Monte Carlo methods.

==> pgfplotsoptions.tex <==
%% create a new cycle list for egsz plots
\pgfplotscreateplotcyclelist{egsz color}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black, mark size=1pt}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black, mark size=1pt},  mark=square*},
  {brown!60!black,every mark/.append style={fill=brown!90!black, mark size=1pt},mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black, mark size=1pt},mark=otimes*},
}

\pgfplotscreateplotcyclelist{egsz color twocol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black!30}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black!30},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!70!black!30},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz bw twocol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!15}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!15},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!15},mark=triangle*},
}
  
\pgfplotscreateplotcyclelist{egsz color threecol}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=diamond*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=diamond*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=triangle*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=triangle*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=triangle*},
  {blue!60!black, every mark/.append style={fill=blue!80!black},    mark=square*},
  {red!60!black,  every mark/.append style={fill=red!80!black},     mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},   mark=square*},
  }

\pgfplotscreateplotcyclelist{egsz bw threecol}{%
  {black, every mark/.append style={fill=black},    mark=*},
  {black, every mark/.append style={fill=black!35}, mark=*},
  {black, every mark/.append style={fill=black!5}, mark=*},
  {black,  every mark/.append style={fill=black},     mark=diamond*},
  {black,  every mark/.append style={fill=black!35},  mark=diamond*},
  {black,  every mark/.append style={fill=black!5},  mark=diamond*},
  {black,every mark/.append style={fill=black},   mark=triangle*},
  {black,every mark/.append style={fill=black!35},mark=triangle*},
  {black,every mark/.append style={fill=black!5},mark=triangle*},
  {black,every mark/.append style={fill=black},   mark=square*},
  {black,every mark/.append style={fill=black!35},mark=square*},
  {black,every mark/.append style={fill=black!5},mark=square*},
}  
  
\pgfplotscreateplotcyclelist{egsz color comparison}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black!50}, mark=square*},
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=diamond*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=triangle*},
}

\pgfplotscreateplotcyclelist{egsz color mi}{%
  {blue!60!black, every mark/.append style={fill=blue!80!black}, mark=*},
  {red!60!black,  every mark/.append style={fill=red!80!black},  mark=square*},
  {green!30!black,every mark/.append style={fill=green!50!black},mark=diamond*},
}

\pgfplotscreateplotcyclelist{egsz bw mi}{%
  {black, every mark/.append style={fill=black}, mark=*},
  {black,  every mark/.append style={fill=black!35},  mark=square*},
  {black,every mark/.append style={fill=black!5},mark=diamond*},
}

%% set styles for general plots and error plots
\pgfplotsset{
  /tikz/tikzpic options/.style={
    scale=0.8,
  },
  egm plot/.style={
    thin, % very thin, thin, semithick, thick, very thick
    %rounded corners=3pt,
    label style={font=\footnotesize}, %\tiny, \scriptsize, \footnotesize
    width=0.65\textwidth,
    height=0.3\textheight,
    grid=major, % none, major, minor, both
    legend columns=1,
    legend pos=south west,
    legend style={font=\tiny, rounded corners=2pt, cells={anchor=west}},
  },
  zmeancoverr plot/.style={
    egm plot,
    xlabel={number of nodes for $r\in(0, 10]$},
    xlabel style={yshift=0.em},
    ylabel={relative $\ell^2$ error},
    legend columns=1,
    %xmin=0.08,
    %xmax=1.5,
    %restrict x to domain=0.08:1.5,
    legend pos=north east,
    cycle list name=egsz color,
    %every axis plot/.append style=only marks,
  },
    zmeancoverrCalls plot/.style={
    egm plot,
    xlabel={number of posterior calls},
    xlabel style={yshift=0.em},
    ylabel={relative $\ell^2$ error},
    legend columns=2,
    %xmin=0.08,
    %xmax=1.5,
    %restrict x to domain=0.08:1.5,
	legend style={at={(0.5,1.05)},anchor=south},
    cycle list name=egsz color,
    %every axis plot/.append style=only marks,
  },
    zmeancoverrCallsLeft plot/.style={
    egm plot,
    width=0.55\textwidth,
    xlabel={number of posterior calls},
    xlabel style={yshift=0.0em},
    ylabel={relative $\ell^2$ error},
    legend columns=1,
    %xmin=0.08,
    %xmax=1.5,
    %restrict x to domain=0.08:1.5,
	legend style={at={(0.2,0.1)},anchor=south},
    cycle list name=egsz color,
    %every axis plot/.append style=only marks,
  },
    zmeancoverrCallsRight plot/.style={
    egm plot,
    width=0.55\textwidth,
    xlabel={number of posterior calls},
    xlabel style={yshift=0.0em},
    ylabel={},
    legend columns=0,
    %xmin=0.08,
    %xmax=1.5,
    %restrict x to domain=0.08:1.5,
	legend style={at={(0.5,1.05)},anchor=south},
    cycle list name=egsz color,
    %every axis plot/.append style=only marks,
  },
  zmeancoverrCallsQuad plot/.style={
    egm plot,
    width=0.55\textwidth,
    xlabel={number of posterior calls},
    xlabel style={yshift=0.0em},
    legend columns=1,
    legend style={at={(0.2,0.1)},anchor=south},
    cycle list name=egsz color,    
  },
  zmeancoverrCallsQuada plot/.style={
     zmeancoverrCallsQuad plot,
	 ylabel={relative $\ell^2$ error},
  },
  zmeancoverrCallsQuadb plot/.style={
     zmeancoverrCallsQuad plot,
	 ylabel={},
  },
}

\tikzset{slopetriangle/.style={
    bottom color=black!20,
    middle color=black!5,
    top color=white,
    draw=black}
    }

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End: 

